Optimal Robust Learning of Discrete Distributions from Batches

Many applications, including natural language processing, sensor networks, collaborative filtering, and federated learning, call for estimating discrete distributions from data collected in batches, some of which may be untrustworthy, erroneous, faulty, or even adversarial. Previous estimators for this setting ran in exponential time, and for some regimes required a suboptimal number of batches. We provide the first polynomial-time estimator that is optimal in the number of batches and achieves essentially the best possible estimation accuracy.

==> preamble.tex <==
\usepackage{makecell}
\usepackage{bbm}
%\usepackage{cite}
\usepackage{epsfig}
\usepackage{latexsym}
\usepackage{setspace}
\usepackage{flushend}
\usepackage{authblk}
%\usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}
\usepackage{float}
\usepackage{dsfont}
%\usepackage{comment}
\usepackage{ upgreek }
\usepackage{caption}
%\usepackage[backref,colorlinks,citecolor=blue,bookmarks=true]{hyperref}
\usepackage{stmaryrd}
\usepackage{xspace}
%\usepackage{algorithm,algorithmic}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage{url}
\usepackage{amsmath,amssymb,amsfonts,amsthm,color,xspace}
\usepackage{graphicx,tikz,enumitem}
\usepackage{verbatim}

%\usepackage{algorithm}% http://ctan.org/pkg/algorithm
%\usepackage{algpseudocode}

%%\newcommand{\theHalgorithm}{\arabic{algorithm}}
%%\usepackage[boxed,titlenotnumbered]{algorithm2e}

\usepackage[preprint,nonatbib]{neurips_2019}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
%\RequirePackage{natbib}
%\setcitestyle{authoryear,round,citesep={;},aysep={,},yysep={;}}

%\newcommand{\yrcite}[1]{\citeyearpar{#1}}
%\renewcommand{\cite}[1]{\citep{#1}}

\usepackage[utf8]{inputenc}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting      % 
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.





%\renewenvironment{comment}{}{}

%% Custom commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Environment
\newcommand{\ba}{\begin{align}}
\newcommand{\ea}{\end{align}}
\newcommand{\ban}{\begin{align*}}
\newcommand{\ean}{\end{align*}}
\newcommand{\lbl}[1]{\label{}}

\newcommand{\br}{\begin{remark}}
\newcommand{\er}{\end{remark}}


%% Brackets

\newcommand{\lc}{\left(}
\newcommand{\rc}{\right)}
\newcommand{\ls}{\left[}
\newcommand{\rs}{\right]}
\newcommand{\lcr}{\left\{}
\newcommand{\rcr}{\right\}}

%% Probabilities
\newcommand{\dR}{\mathrm{R}}
\newcommand{\dP}{\mathrm{P}}
\newcommand{\dQ}{\mathrm{Q}}
\newcommand{\dPr}{\mathbb{P}}
\newcommand{\bP}[2]{\mathrm{P}_{#1}\left(#2\right)}
\newcommand{\bQ}[2]{\mathrm{Q}_{#1}\left(#2\right)}
\newcommand{\bPP}[1]{\mathrm{P}_{#1}}
\newcommand{\bQQ}[1]{\mathrm{Q}_{#1}}
\newcommand{\bRR}[1]{\mathrm{R}_{#1}}
\newcommand{\bPr}[1]{\dPr\left(#1\right)}
\newcommand{\tPr}[1]{\tilde{\mathrm{P}}\left(#1\right)}
\newcommand{\tPP}[1]{{\tilde{\mathrm{P}}}_{#1}}
\newcommand{\tP}[2]{\tilde{\mathrm{P}}_{#1}\left({#2}\right)}
\newcommand{\tPs}[3]{\tilde{\mathrm{P}}^{#1}_{#2}\left({#3}\right)}
\newcommand{\bE}[2]{{\mathbb{E}}_{#1}\left[{#2}\right]}
\newcommand{\bEE}[1]{{\mathbb{E}}\left[#1\right]}
\newcommand{\mcf}{\mathrm{mcf}}

\newcommand{\popt}{p^{\text{opt}}}

\renewcommand{\atop}[2]{\genfrac{}{}{0pt}{1}{#1}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}


\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem*{remarks*}{Remarks}


\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\qedsymbol}{\ensuremath{\blacksquare}}

%% undertilde %%
\def\undertilde#1{\mathord{\vtop{\ialign{##\crcr
$\hfil\displaystyle{#1}\hfil$\crcr\noalign{\kern1.5pt\nointerlineskip}
$\hfil\tilde{}\hfil$\crcr\noalign{\kern1.5pt}}}}}



% greek %
\newcommand{\ep}{\varepsilon}
\newcommand{\la}{\lambda}


% latex %
\newcommand{\nn}{\nonumber}
\newcommand{\ds}{\displaystyle}
\renewcommand{\atop}[2]{\genfrac{}{}{0pt}{1}{#1}{#2}}
%\newcommand{\hilight}[1]{\colorbox{yellow}{#1}}
\newcommand{\hilight}[1]{\textcolor{blue}{#1}}

% functionals of distributions %
\newcommand{\ttlvrn}[2]{d_{\mathtt{var}}\left( #1 , #2\right)}
\newcommand{\KL}[2]{D\big( #1 \big\| #2\big)}
\newcommand{\CKL}[3]{D\big( #1 \big\| #2\, \big|\, #3\big)}
\newcommand{\MI}[2]{I\left(#1 \wedge #2\right)}
\newcommand{\CMI}[3]{I\left(#1 \wedge #2\mid #3\right)}
\newcommand{\RDg}{D_\alpha(\dP, \dQ)}

% random variables and properties %
\newcommand{\indicator}{{\mathds{1}}}
\newcommand{\mc}{-\!\!\!\!\circ\!\!\!\!-}


% basic functions %
\newcommand{\argmax}{\mathop{\rm argmax}\limits}
\newcommand{\argmin}{\mathop{\rm argmin}\limits}

\allowdisplaybreaks
\setlength{\belowcaptionskip}{-0.6cm}


% local commands %

\newcommand{\prot}{\pi}
\newcommand{\Prot}{\Pi}
\newcommand{\protr}{\tau}
\newcommand{\Pprot}{\Pi \Pi}
\newcommand{\simm}{\mathtt{sim}}
\newcommand{\DE}{\mathtt{DE}}
\newcommand{\psim}{\prot_{\simm}} 
\newcommand{\Psim}{\Prot_{\simm} }
\newcommand{\pcom}{\prot_{\mathtt{com}} }
\newcommand{\Pcom}{\Prot_{\mathtt{com}} }
\newcommand{\pdex}{\prot_{\DE}}
\newcommand{\Pdex}{\Prot_{\DE}}
\newcommand{\pmix}{\prot_{\mathtt{mix}}}
\newcommand{\pmixn}{\prot_{\mathtt{mix,n}}}
\newcommand{\Protx}{\Prot_{\cX}}
\newcommand{\Proty}{\Prot_{\cY}}


\newcommand{\dc}[1]{D_\ep\left(#1\right)}
\newcommand{\dcp}{\dc {\prot}}
\newcommand{\dcpp}{\dc {\prot| \bPP{XY}}}


\newcommand{\rmax}{r_{\max}}
\newcommand{\ic}{\mathtt{ic}}
\newcommand{\IC}{\mathtt{IC}}
\newcommand{\icpp}{\ic(\protr; x,y)}
\newcommand{\icp}{\ic(\Prot; X,Y)}
\newcommand{\Icp}{\IC(\prot)}
\newcommand{\varp}{\mathtt{V}(\prot)}

\newcommand{\hxy}{h(X,Y)}
\newcommand{\hsum}[2]{h\left(#1 \triangle #2\right)}
\newcommand{\hsump}{\hsum {X\Prot}{Y\Prot}}
\newcommand{\lamin}{\lambda_{\min}}
\newcommand{\lamax}{\lambda_{\max}}
\newcommand{\lamins}[1]{\lamin^{(#1)}}
\newcommand{\lamaxs}[1]{\lamax^{(#1)}}
\newcommand{\den}{\zeta}

%\newcommand{\epsmall}{\ep_{\mathtt{ngl}}}
\newcommand{\epsmall}{\ep^\prime}
\newcommand{\eptail}{\ep_{\mathtt{tail}}}
%\newcommand{\lasmall}{\la_{\mathtt{ngl}}}
\newcommand{\lasmall}{\la^\prime}

\newcommand{\Hmin}{H_{\min}}
\newcommand{\supp}{\mathtt{supp}}

\newcommand{\Esim}{\cE_{\simm}}
\newcommand{\EDE}{\cE_{\DE}}

\newcommand{\partyx}{Party 1\xspace}
\newcommand{\partyy}{Party 2\xspace}

\newcommand{\prots}{\boldsymbol{\prot}}
\newcommand{\sIcp}{\overline{\mathtt{IC}}(\boldsymbol{\prot}) }

\newcommand{\Order}{\cO}
\newcommand{\order}{o}
\newcommand{\tOrder}{\tilde{\cO}}

\newcommand{\tcb}[1]{\textcolor{blue}{#1}}


% Distributions
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Bin}{\mathrm{Bin}}

% Abbreviation

\newcommand{\whp}{w.h.p.\xspace}


% 
\newcommand{\btotal}{m}
\newcommand{\alphsize}{k}
\newcommand{\alphabet}{[\alphsize]}
\newcommand{\bsize}{n}

\newcommand{\advfrac}{\beta}
\newcommand{\goodfrac}{\alpha}
\newcommand{\allbatches}{{B}}
\newcommand{\bgood}{\allbatches_G}
\newcommand{\badv}{\allbatches_A}

\newcommand{\Bsc}{\allbatches^\prime}
\newcommand{\Gsc}{\allbatches^\prime_G}
\newcommand{\Asc}{\allbatches^\prime_A}

\newcommand{\size}[1]{|{#1}|}

\newcommand{\bgoodsize}{\size{\bgood}}
\newcommand{\badvsize}{\size{\badv}}
\newcommand{\sizeBsc}{\size{\Bsc}}
\newcommand{\sizeGsc}{\size{\Gsc}}
\newcommand{\sizeAsc}{\size{\Asc}}

\newcommand{\alphsubset}{S}
\newcommand{\alphsubsetdef}{ \alphsubset \subseteq \alphabet}


\newcommand{\probestbatch}{\targetdis_b}
\newcommand{\probestbatchsub}{\bar{\targetdis}_b(\alphsubset)}

\newcommand{\targetdis}{p}
\newcommand{\batchdis}{p_b}
\newcommand{\targetdistance}{\eta}


\newcommand{\empdistribution}{\bar \targetdis}

\newcommand{\medV}{\text{med}}
\newcommand{\med}{\text{med}(\bar{\mu}(\alphsubset))}

\newcommand{\estdis}{\targetdis*}

 
\newcommand{\subsetcountbatch}{n_b(\alphsubset)}
%consider changing it to just subsetcount

\newcommand{\subsetprobtarget}{\targetdis(\alphsubset)}
%consider changing it to just subsetprob


\newcommand{\Bempprob}{{\bar{\targetdis}_{\allbatches}(\alphsubset)}}
\newcommand{\Uempprob}{{\bar{\targetdis}_{\Bsc}(\alphsubset)}}
\newcommand{\UGempprob}{{\bar{\targetdis}_{\Gsc}(\alphsubset)}}
\newcommand{\UAempprob}{{\bar{\targetdis}_{\Asc}(\alphsubset)}}
\newcommand{\bempprob}{{\bar{\mu}_{b}(\alphsubset)}}

\newcommand{\VUempprob}{{\bar{\targetdis}_{\Bsc}}}
\newcommand{\VUGempprob}{{\bar{\targetdis}_{\Gsc}}}
\newcommand{\VUAempprob}{{\bar{\targetdis}_{\Asc}}}
\newcommand{\Vbempprob}{{\bar{\mu}_{b}}} %previously  probestbatchsub

\newcommand{\empprobsub}[1]{\bar{\targetdis}_{#1}(\alphsubset)}
\newcommand{\empprob}[1]{\bar{\targetdis}_{#1}}
\newcommand{\empprobsubtotal}{\bar{\targetdis}_{[\btotal]}(\alphsubset)}


\newcommand{\empvarsub}[1]{\overline{\text{V}}_{#1}(\alphsubset)}

\newcommand{\finaldis}{\targetdis^*}

\newcommand{\var}[1]{\text{V}(#1)}

\newcommand{\corruption}{\psi}
\newcommand{\indcorruption}{\corruption_b(\alphsubset)}
\newcommand{\genoverallcorruptionsub}{\corruption(\Bsc,\alphsubset)}
\newcommand{\genoverallcorruption}{\corruption(\Bsc)}

%distribution


%distance
\newcommand{\Lone}{L_1}
\newcommand{\dlone}[1]{||#1||_1}

%useful distances
\newcommand{\optdistance}{\frac \advfrac {\sqrt{\bsize}} }

